Reactive Navigation under Non-Parametric Uncertainty through Hilbert Space Embedding of Probabilistic Velocity Obstacles

The probabilistic velocity obstacle (PVO) extends the concept of velocity obstacle (VO) to work in uncertain dynamic environments. In this paper, we show how a robust model predictive control (MPC) with PVO constraints under non-parametric uncertainty can be made computationally tractable. At the core of our formulation is a novel yet simple interpretation of our robust MPC as a problem of matching the distribution of PVO with a certain desired distribution. To this end, we propose two methods. Our first baseline method is based on approximating the distribution of PVO with a Gaussian Mixture Model (GMM) and subsequently performing distribution matching using Kullback Leibler (KL) divergence metric. Our second formulation is based on the possibility of representing arbitrary distributions as functions in Reproducing Kernel Hilbert Space (RKHS). We use this foundation to interpret our robust MPC as a problem of minimizing the distance between the desired distribution and the distribution of the PVO in the RKHS. Both the RKHS and GMM based formulation can work with any uncertainty distribution and thus allowing us to relax the prevalent Gaussian assumption in the existing works. We validate our formulation by taking an example of 2D navigation of quadrotors with a realistic noise model for perception and ego-motion uncertainty. In particular, we present a systematic comparison between the GMM and the RKHS approach and show that while both approaches can produce safe trajectories, the former is highly conservative and leads to poor tracking and control costs. Furthermore, RKHS based approach gives better computational times that are up to one order of magnitude lesser than the computation time of the GMM based approach.

==> chapters/limitations.tex <==
\subsection{Limitations of the proposed method}
Our formulations can fail due to two reasons. First, there can be a failure in construction of the desired distribution if no feasible solution exists for the optimization problem proposed in (\ref{cost_scenario})-(\ref{feasible_scenario}). Second, if the control sampling is not dense enough and we miss some out on some feasible control inputs.  The latter can be handled by increasing the resolution of discretization of control inputs, although this would lead to an increase in computation time.


==> chapters/multi-agent.tex <==
\subsection{Extensions to multiple moving objects}
To extend the proposed formulation to a multi-agent system, we propose that $f_t^j$ represents the analytical form of the Reciprocal velocity obstacle (RVO) mentioned in \cite{prvo}, \cite{air-bharath}. We replace the VO constraints by RVO to ensure that the executed trajectories are oscillation free \cite{rvo} \cite{orca}.

We propose the following steps that capture the critical changes required to construct a robust MPC scheme that achieves multi-agent collision avoidance under non-parametric uncertainty.

\begin{itemize}
    \item The deterministic constraint on velocity obstacle (\ref{vo}), would now be changed to that of the RVO \cite{prvo}\cite{air-bharath}.
    
    \item Accordingly, the only change in the steps mentioned for constructing the desired distribution (refer Appendix \ref{sec:appendix-desired-distribution}), would be to derive the function in (\ref{scenario_const}) according to the analytical form of the RVO constraint.
    
    \item The rest of the steps that are involved in the current chance-constrained formulation (\ref{compact_vo})-(\ref{eq:reduced-set}), along with the assumptions on non-parametric uncertainty (refer Fig. \ref{fig:error-distributions}), would essentially remain the same.
\end{itemize}
